Stay Tuned: An Empirical Study of the Impact of Hyperparameters on LLM Tuning in Real-World Applications

Fine-tuning Large Language Models (LLMs) is an effective method to enhance their performance on downstream tasks. However, choosing the appropriate setting of tuning hyperparameters (HPs) is a labor-intensive and computationally expensive process. Here, we provide recommended HP configurations for practical use-cases that represent a better starting point for practitioners, when considering two SOTA LLMs and two commonly used tuning methods. We describe Coverage-based Search (CBS), a process for ranking HP configurations based on an offline extensive grid search, such that the top ranked configurations collectively provide a practical robust recommendation for a wide range of datasets and domains. We focus our experiments on Llama-3-8B and Mistral-7B, as well as full fine-tuning and LoRa, conducting a total of > 10,000 tuning experiments. Our results suggest that, in general, Llama-3-8B and LoRA should be preferred, when possible. Moreover, we show that for both models and tuning methods, exploring only a few HP configurations, as recommended by our analysis, can provide excellent results in practice, making this work a valuable resource for practitioners.

==> analysis_bar_charts.tex <==
\begin{figure*}
    \centering
    \subfigure[]{\includegraphics[width=0.3\linewidth]{latex/Figures/Screenshot 2024-07-14 at 15.49.51.png}}
    \subfigure[]{\includegraphics[width=0.3\linewidth]{latex/Figures/Screenshot 2024-07-14 at 15.48.10.png}}
    \subfigure[]{\includegraphics[width=0.3\linewidth]{latex/Figures/Screenshot 2024-07-14 at 15.51.06.png}}
    % \caption{Hyper-parameter distribution patterns. (a) Relatively even distribution of the effective batch size, doing full fine-tuning on classification datasets using 1000 training examples with Mistral-7B-v0.3. (b) Distribution of learning rate dominated by a sub-set of the possible values, doing full fine-tuning on CQA datasets using 100 training examples with Llama-3-8B. (c) Mixed distribution of learning rate, doing full fine-tuning on classification datasets using 1000 training examples with Mistral-7B-v0.3. }
    \caption{Hyper-parameter distribution patterns. (a) Relatively even distribution, (b) Distribution dominated by a sub-set of the possible values, (c) Mixed distribution.}  \red {Figure is too small.}
   \label{fig:hp_bar_charts}
\end{figure*}

\begin{figure*}[ht]
\begin{center}
\includegraphics[width=0.9\textwidth]{latex/Figures/full-ft-heatmap-2.png}
\caption{Heat map of $JSpval(hp)$ values. Low (dark) scores indicate larger distribution variance between datasets.}
\label{fig:full_ft_heatmap}
\end{center}
\end{figure*}

==> gain_upper_bound_results_tables.tex <==
% \begin{table*}[!ht]
%     \centering
%     \resizebox{\textwidth}{!}{%
%     \begin{tabular}{l|l|l|l|l|l|l|l|l|}
%     \hline
%         & \multicolumn{4}{c}{Llama-3-8B} &
%         \multicolumn{4}{c}{Mistral-7B-v0.3} \\ \hline
%         & \multicolumn{2}{c}{Full-FT} & \multicolumn{2}{c}{LoRA} & \multicolumn{2}{c}{Full-FT} & \multicolumn{2}{c}{LoRA} \\ \hline
%         ~ & 100 & 1000 & 100 & 1000 & 100 & 1000 & 100 & 1000 \\ \hline
%         Classification & 73.36 (4.3) & 81.53 (1.8) & 74.43 (5.8) & 81.84 (1.6) & 69.03 (5.4) & 70.63 (2.6) & 78.66 (12.1) & 79.54 (6.5) \\ \hline
%         Summarization & 28.27 (0.8) & 29.18 (1.3) & 28.73 (0.4) & 28.82 (0.2) & 27.95 (1.3) & 29.27 (0.4) & 27.91 (0.9) & 28.17 (0.3) \\ \hline
%         CQA & ~ & ~ & ~ & ~ & ~ & ~ & ~ \\ \hline
%     \end{tabular}
%     }
%     \caption{\red{Update Table} Results when doing dataset-specific hyper-paramter tuning. In parenthesis are the gains compared to using the best task hyper-parameter recommendation (Table~\ref{tab:recommendations_table}). Scores are averaged over all datasets for the given task. We report micro-f1 for classification and rougeL for summarization and CQA. \red{check}}
%     \label{tab:gains_over_recommendations}
% \end{table*}

==> lora_vs_full.tex <==
\begin{table}[]
\centering
\resizebox{\columnwidth}{!}{%
\begin{tabular}{llllllll}
Model name & task type & train size & Best full FT & LOO full FT & Best LORA & LOO LoRA & best-baseline \\
\hline
Llama   & Classification & 100 & 88 & 84 & 86 & 80 & 5 \\
Llama   & Summarization  & 100 & 88 & 84 & 86 & 80 & 5 \\
Llama   & CQA            & 100 & 88 & 84 & 86 & 80 & 5 \\
\hline
Mistral & Classification & 100 & 88 & 84 & 86 & 80 & 5 \\
Mistral & Summarization  & 100 & 88 & 84 & 86 & 80 & 5 \\
Mistral & CQA            & 100 & 88 & 84 & 86 & 80 & 5 \\
\end{tabular}%
}
\caption{
Table for contribution 2: Comparison between full FT and LoRA on their best and LOO setting
}
\end{table}


==> old_analysis.tex <==

\section{Analysis}

In the previous section we have established task-level recommendations for hyper-tuning in diverse, real-world scenarios. We also provided support for the need for dataset-specific hyperparameter tuning in certain cases. Still, in doing so it could be beneficial to understand if there are hyper-parameters that are more important to finetune than others.

\subsection{Hyper-parameter tuning prioritization}

In order to address this question, we suggest to measure how the distribution of values of each hyperparameter varies between the datasets. Finetuning parameters with higher variability between the datasets is likely to yield higher performance gains over the globally recommended parameter value.   

To this end, we define for each task, model, tuning method and number of training examples, the set of \emph{top} hyper-parameter configurations $TC$ in each dataset $d$ as:

\[
TC = \{\mathbf{c} \in \mathcal{S} \mid s(c) > 0.95 * \max_{\mathbf{c} \in \mathcal{S}} s(\mathbf{c})\}
\]

\red{yk - reviewer may ask why 95 precent there and 97 percent threshold before}
where $\mathcal{S}$ is the set of all possible configurations and $s(\mathbf{c})$ is the score obtained by using configuration $\mathbf{c}:=(c_1,...,c_k)$ on $d$.

Then, for each hyper-parameter $i$ and possible hyper-parameter value $v$, we calculate its relative frequency in $TC$:

\[
p(c_i=v) = \frac{|\{\mathbf{c} \in TC|c_i=v\}|}{|TC|}
\]

This allows us to obtain a probability vector $\mathbf{p_{i,d}}$ for each hyper-parameter $i$ and dataset $d$, with the probabilities calculated over all possible values the $i$th parameter in $\mathcal{S}$.

\input{latex/analysis_bar_charts}

The resulting probability vectors could be either evenly distributed across all possible hyper-parameter values; dominated by a sub-set of the values; or mixed between the values. Examples for each of these patterns are presented in Figure~\ref{fig:hp_bar_charts}.

Specifically, we look for those hyper-parameters which are more unexpected when moving from one dataset to another, i.e., produce more varied probability vectors. For this purpose we define:

\[
JSScore(hp) = \\
\]
\[
1-\frac{\sum_{p1,p2 \in P, p1 \neq p2} JDdist(p1,p2)}{{|P| \choose 2}}
\]

Where $P$ is the list of probability vectors (one for each dataset), and $JSDist$ is the jensen-shannon distance.

To assess the significance of the $JSScore(hp)$ values we conduct the following permutation test \cite{fisher:1935}: We obtain $100$ permutations of $TC$ where in each permutation we assign a random mapping of configurations to datasets. We then use these permutations to calculate the following:

\[
JSpval(hp) = \\
\]
\[
\frac{|JSScore(hp)<JSScore^i(hp) _{0\leq i \leq100}|}{100}
\]

In other words, we calculate how many permutations entail distributions which are less diverse than the observed distribution. A low $JSpval$ value indicates that the observed distribution is meaningful, rather than obtained at random.

We plot a heatmap of all $JSpval$ values for full fine-tuning experiments in Figure~\ref{fig:full_ft_heatmap}.

